Combining Latent Space and Structured Kernels for Bayesian Optimization over Combinatorial Spaces

We consider the problem of optimizing combinatorial spaces (e.g., sequences, trees, and graphs) using expensive black-box function evaluations. For example, optimizing molecules for drug design using physical lab experiments. Bayesian optimization (BO) is an efficient framework for solving such problems by intelligently selecting the inputs with high utility guided by a learned surrogate model. A recent BO approach for combinatorial spaces is through a reduction to BO over continuous spaces by learning a latent representation of structures using deep generative models (DGMs). The selected input from the continuous space is decoded into a discrete structure for performing function evaluation. However, the surrogate model over the latent space only uses the information learned by the DGM, which may not have the desired inductive bias to approximate the target black-box function. To overcome this drawback, this paper proposes a principled approach referred as LADDER. The key idea is to define a novel structure-coupled kernel that explicitly integrates the structural information from decoded structures with the learned latent space representation for better surrogate modeling. Our experiments on real-world benchmarks show that LADDER significantly improves over the BO over latent space method, and performs better or similar to state-of-the-art methods.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
  \answerYes{}
  \item Did you describe the limitations of your work?
\answerYes{We discussed potential limitation in Section 6.}

  \item Did you discuss any potential negative societal impacts of your work?
  
 \answerYes{Since LADDER is a general expensive black-box optimization algorithm, it's social impact is determined by the nature of end-application it is employed in and the optimization objective for a particular application. For example, accelerating the design of drugs/vaccines vs. gain of function experimental selection.}
  
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
  \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
 \answerNA{}
	\item Did you include complete proofs of all theoretical results?
 \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
  
   \answerYes{We provide our code in the supplementary material and a thorough description of the experimental setup is given in Section 4.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
  
 \answerYes{All the training details are given in Section 4.2.}

    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
	
\answerYes{We show the error bars in all our figures.}
	
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
	\answerYes{we provide the details of the computing resource used for our experiments in Section 4.2.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
  
  \answerYes{We cited the original authors' for code libraries and datasets that we used in Section 4.}
  \item Did you mention the license of the assets?
  
  \answerYes{The license is kept in the supplementary material.}
  
  \item Did you include any new assets either in the supplemental material or as a URL?
  
  \answerYes{We added our own Bayesian optimization code in the supplementary material.}

  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
  
  \answerYes{We use all open-source codes available on public Github repositories.}
  
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
  \answerNA{}

\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?  N/A
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?  
    \answerNA{}
  
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation? 
    \answerNA{}
\end{enumerate}

\end{enumerate}
